Leveraging WiFi Network Logs to Infer Student Collocation and its Relationship with Academic Performance

A comprehensive understanding of collocation can help understand performance outcomes. For university cohorts, this needs data that describes large groups over a long period. Harnessing user devices to infer this, while tempting, is challenged by privacy concerns, power consumption, and maintenance issues. Alternatively, embedding new sensors in the environment is limited by the expense of covering the entire campus. We investigate the feasibility of leveraging WiFi association logs for this purpose. While these provide coarse approximations of location, these are easily obtainable and depict multiple users on campus over a semester. We explore how these coarse collocations are related to individual performance. Specifically, we inspect the association between individual performance and the collocation behaviors of project group members. We study 163 students (in 54 project groups) over 14 weeks. After describing how we determine collocation with the WiFi logs, we present a study to analyze how collocation within groups relates to a student's final score. We find collocation behaviors show a significant correlation (Pearson's r = 0.24) with performance -- better than both peer feedback or individual behaviors like attendance. Finally, we discuss how repurposing WiFi logs can facilitate applications for domains like mental wellbeing and physical health.

==> 061.tex <==
\section{Other Uses of Archival Network Logs}
\edit{Our study demonstrates }
that infrastructure-based coarse collocation captures some important aspects of social behaviors in students, 
which can be predictors of group project success.
This presents new opportunities to harness archival network logs to scale analyses of social behaviors for larger groups, up to and including an entire campus. For instance, with an empirical understanding of how successful teams socially interact, instructors can tailor recommendations for project courses.
\edit{This section illustrates other potential use-cases to harness these logs for assessing long-term social behaviors at scale.}

\subsection{Interaction Networks}
\label{sec:applications_interaction}
\edit{
The collocation inferred from these logs can be used to develop social networks representing an entire campus community. }
This use-case is similar to what \citeauthor{hong2016socialprobe}, describe as relationship maps to understand intimacy between individuals~\cite{hong2016socialprobe}. 
\edit{Since these logs can be archived for long periods of time it is possible to study the development and evolution of these social networks.
}
Moreover, by contextualizing these collocations based on when and where these interactions happen it can help study multiplexed social networks for different purposes 
(e.g., residential ties for roommates, academic ties for project teams, or recreational ties for parties). Accordingly, stakeholders can consider reactive actions to secure cohorts when they notice anomalies in a network, such as when someone from a cohort drops out, is affected by an mental trauma (e.g., violent incident), or is physically unwell (e.g., contagious disease)---the campus can react by securing the peers first.

\subsection{Interaction Spaces}
\label{sec:applications_space}
\edit{These logs can also help describe the utilization of spaces for social purposes.
Even retrospective analysis of the data can describe where students congregate before exam week, or if certain weeks of a semester observe more parties.
}
This would require collaborating with community stakeholders who understnad the ground reality of the space and can contextualize such insights. 
Accordingly administrators could focus on facilitating better interaction in these spaces during times of collaboration. By contrast, they could also choose to carefully regulate the use of these spaces during times of social distancing~\cite{martin2020effectiveness}. 

\subsection{Congestion Patterns}
\label{sec:application_congestion}
% \munmun{Simply call this mobility? Maybe spatio-temporal mobility?}
% From the perspective of mental wellbeing, physical social interactions are considered constructive, however in many cases of physical wellbeing they are considered detrimental. 
Social interactions in physical spaces can lead to congestion depending on the purpose and popularity of a space. Understanding where these spaces are and when  congestion can occur can regulate gatherings for crowd-management~\cite{fan2015citymomentum,wang2016crowdwatch} and even prevent the spread of contagious diseases~\cite{martin2020effectiveness}.
% \thomas{I am confused by that last sentence, it seems contradictory in itself?} 
Therefore, campus stakeholders have an interest in identifying rooms and pathways with high pedestrian concentration. 
\edit{While this study primarily focuses on dwelling, it would be possible to study the phases when people move together, e.g., between classes.}
Not only could this help pre-determine bottle-necks for flock movement in cases of emergencies, it can also retroactively indicate which spaces were prone to congestion and inadvertent physical contact. 

% based on insights gathered from the case study.

% Unlike invasive client-based localization techniques,
% Since this method relies on logs, it can harness archival data for retrospective analyses in a way that client deployments cannot.

% \thomas{Ok, so the advantage of infrastructure-based sensing is not new and something we would need to sell here.} 

% While the method proposed in this paper does not provide the precision of fingerprinting methods it is less resource intensive because it does not require an extensive training phase \thomas{Well, we did train regression models, no?}. Traditional fingerprinting would require every building, containing multiple floors and rooms to be mapped for signal strength. Add to that the consideration of the dynamic objects that could potentially alter the signal strength  (e.g., people, new devices, solid objects). By contrast, our method provides a coarse notion of presence or proximity to an access point which is further extended to a coarse notion of co-presence. In fact, this information can reveal behaviors that indicate social interactions among individuals connected to the network. This section describes some of the applications of this that we could validate based on the ground-truth. \thomas{"could"?}





% \mehrab{general comment about this subsection. Sequencing problem for figures: figure 13 comes before firgure 12. In addition, do mention what was used to construct the network graphs. IMWUT reviewers generally ask for this kind of tool-centric details.}
% \label{sec:applications_interaction}
% Social interactions are crucial to understand the physical and mental wellbeing of an individual. The lack of social interaction, or social isolation, is linked to stress, negative affect, depression and dissatisfaction~\cite{skek1991life,finch1997factor,ford1990relationship}.
% \thomas{Wow, that's quite a jump!} 
% The presence of social interactions can uncover ties within a peer group, which can be helpful to understand individual perception and behavior. For instance, weak social ties are related to a lack of motivation to go to work or absenteeism~\cite{unden1996social}. Alternatively, strong social ties can also explain peer influence and its effect on alcohol, drug and tobacco use~\cite{crosnoe2004childhood}.
% also be used to infer homophily in groups which can represent congruence in perceptions and behaviors~\cite{XX}. 
% For instance, an individual can be motivated towards an activity based on their close group of associates. 
% In terms of physical wellbeing, groups with dense social interactions have increased risk of spreading contagious diseases~\cite{}. 
% As a result, retrospective investigations of who a student interacts with and how these interactions evolve over a period of time can provide insights for supporting student wellbeing.

% \begin{figure}[t]
%     \begin{minipage}[t!]{1\columnwidth}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/network_jdb_2.png}
%       \caption{1st week of class}
%           \label{fig:net_2}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/network_jdb_8.png}
%       \caption{Mid-term}
%           \label{fig:net_8}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/network_jdb_12.png}
%       \caption{12th week}
%           \label{fig:net_12}
%         \end{subfigure}
%         \caption{Network graph representing time spent between individuals of 1B}
%         % \thomas{Why are these results not in the results section but in this applications section?}}
%         \label{fig:net_weekly}
%     \end{minipage}\hfill
% \end{figure}

% \begin{wrapfigure}{r}{0.35\textwidth}
%   \begin{center}
%     \includegraphics[width=0.35\textwidth]{figures/network_jid_agg.png}
%   \end{center}
%   \caption{Network graph representing collocation time (outside class) for individuals of section 2D aggregated over the semester}
%     \label{fig:net_agg}
%     \vspace{-0.15in}
% \end{wrapfigure}



% Using the data from Section~\ref{sec:main-case-study}, we develop network graphs representing the collocation between pairs of individuals in the same section, shown in Figure~\ref{fig:net_weekly}. We compute the graphs  week-wise (excluding lecture times), with each edge depicting the duration of collocation between any pair of individuals. 
% % The graphs were limited to students in the same section of a class and . 
% Figure~\ref{fig:net_weekly} shows the evolution of these interaction ties between participants from Section 1B. Every node represents a participant and the color denotes project groups. Nodes that are closer illustrate individuals who spent more time collocated together.
% % The distance between nodes is indirectly proportional to the duration two individuals were collocated together over that week. 
% Even in the first week of class, the participants are somewhat closer to their group members than others, and this becomes more pronounced in the later weeks. However, since we consider all collocations it is evident that a participant's ties are not exclusive to their group. This makes automated methods even more valuable so as to identify these informal interactions. In some cases, members of different groups might be connected through other courses or even social circles. 
% Similarly,  Figure~\ref{fig:net_agg}  represents interaction ties in section 2D aggregated over the whole study period. It reveals  the tight connection amongst some members of the red group. This particularly refers to participants 2006, 2009, and 2010. In comparison, two other group members are slightly further apart. This is explained by the disclosure during enrollment that these participants  live together. 
% Apart from them only four other participants indicated interacting with their group members outside the purposes of the academic objectives. 
% By using raw association logs for an entire campus, 
% it presents opportunities to understand where these interactions occur and semantically labels them based on the expected purpose of collocation 
% Note that our sample is limited to the 215 individuals that consented to the use of their network logs. 
% Yet, through visual analysis of the collocation based network graphs alone one can determine the tie strength between different individuals.  
% More nuanced automated learning techniques can help identify social groups in a completely unsupervised way, making a compelling argument for the application to a broader cohort on campus. 
% Accordingly, stakeholders can take actions for a cohort of individuals based on noticeable anomalies in a network, such as when someone from a cohort drops out. Another use case is when someone in a network is affected by an ailment---mental (e.g., violent incident) or physical (e.g., contagious disease)---the campus can react by securing the peers first.


% \begin{table}[t]
%     \begin{minipage}[t!]{1\columnwidth}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_before.png}
%       \caption{Before}
%           \label{fig:hmap_before}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_during.png}
%       \caption{During}
%           \label{fig:hmap_during}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_after.png}
%       \caption{After}
%           \label{fig:hmap_after}
%         \end{subfigure}
%         \captionof{figure}{Space usage around the midterm}
%   \label{fig:hmap_space}
%     \end{minipage}\hfill
% \end{table}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/space_colloc.png}
%     % \vspace{-0.1in}
%   	\caption{Duration of collocations for part 1 students based on the semantic label of buildings (averaged by week).}
%   	   \label{fig:space_colloc}
%   	      \vspace{-0.35in}
% \end{figure}



% \mehrab{what does it mean to have a 0 hour after midterm in residential buildings?
% Does it indicate that there was no team deliverable after midterm and that's why students did not meet? Can we make any comments on the huge drop?
% Which category CULC or library falls under? Was there any insights for such spaces?}
% \munmun{Space utilization?}

% Another approach to visually analyzing the segments identified by the pipeline is to observe where social interactions occur. 
% On simply observing the patterns of dwelling an analyst can determine where "crowding" occurs or alternatively which spaces show sparse use. 
% Figure~\ref{fig:hmap_space} shows how the dwelling changes before the midterm, during the midterm, after the midterm and in the final week.


 
% This can be further expanded by locating the ``collocation spaces'', which are spots on campus where individuals gather together. ~\autoref{fig:space_colloc} shows how the collocation changes before the midterm, during the midterm, after the midterm. While there is a slight increase in collocation period at academic spaces towards the end of the semester, it is most notable how the interactions in residential spaces change during the midterm. This excessive collocation could indicate groups working together to collaborate on midterm milestones or simply study for exams. Another notable aspect is the decrease of collocation duration at fraternities and sororities. This might be related to fewer parties and gatherings during midterm exams. More importantly, this data provides evidence that social interactions vary over time at different places. 
% By investigating how collocation varies around specific events, say an exam, it is possible to define the purpose of spaces more dynamically. Furthermore, this can be extended to gain a better understanding of the purpose of social interactions itself. 
% \thomas{So, these applications are all well and fine. However, in the absence of actual research questions (unless I am missing something, I only saw one stray hint on a "RQ2", which, however, I believe was never formally introduced) it looks all a bit unstructured. What is it that we are actually trying to research? At the moment it reads a bit like we found a cool technology (which in itself is not brandnew) and are playing around with it to see what we can find out. I know that this is not how we have been working on this project for the last n months, but that's how the paper reads like at the moment. So, my suggestion is to work on the structure of the paper and guide it through explicitly formulated (and motivated) research questions. I have also given suggestions on how to re-organize parts of the paper to make it flow better.}





% This subsection presents some observational evidence from our data showing how sections move in and out of their class room around a lecture.

% \begin{table}[t!]
%     \begin{minipage}[t!]{\columnwidth}
%     % \begin{subfigure}[b]{\columnwidth}
%     %     \centering
%     %     \includegraphics[width=0.7\columnwidth]{figures/lecture_attendance.png}
%     %   \end{subfigure}
%     % \captionof{figure}{Attendance of 1A as detected by dwelling}
%     \label{fig:lecture_attendance}
%     \end{minipage}\hfill
%     \begin{minipage}[t!]{\columnwidth}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=0.9\columnwidth]{figures/lecture_punctuality.png}
%       \end{subfigure}
%     \captionof{figure}{Punctuality of attending students from 1A, where the vertical red dashed lines indicate lecture times}
%     \label{fig:lecture_punctuality}
%     \end{minipage}\hfill
%     \vspace{-0.1in}
% \end{table}

% As discussed in Section~\ref{sec:attendance-validation}, one of the instructors (1Q) provided us with lecture-by-lecture attendance data (46 students in Sections 1A and 1B). For Section 1A, lectures took place three times a week from 10:10-11:00, and for Section 1B, these lectures took place from 11:15-12:05. 
% % In total we compute the presence of individuals for 34 lectures (this excludes the spring break period). For these lectures, over the study period we identify 83\% of students on the network to be connected to the same AP as that associated with the room and 93\% of the students to be connected to an AP in the building. Having said that, throughout the study period about 10\% of the students in the class did not connect to the network infrastructure. 
% The rooms where these lectures took place were both single entry/exit. To gain a better understanding of how congested these points can get, we evaluate the arrival and exit times of the students that attend class. 
% % This can be considered an under-fill/overfill error.
% For entering class, we compare the earliest starting time of an individual's collocation with the designated commencement time. Similarly for exiting class, we compare the latest ending time with the lecture's expected conclusion time. The median entering time is five minutes and the median exiting time is two minutes (Figure~\ref{fig:lecture_punctuality}). These values align with the instructors' observation of typical class behavior, i.e., students are typically tardy on entry but are on time for the exit. 

% Notably, our analysis considers the only students from the current class and not those who would occupy the same room for the next  or previous lecture. However, with richer data, it is possible to understand congestion points not just for class rooms but where any social interactions occur. With these findings, stakeholders could regulate the exit of students even between different rooms to avoid crowding the pathways. These can be proactive interventions to reduce the physical interactions. 
% Additionally, it can be coordinated with the lecture times of neighboring classrooms to allow smoother safer movement. This observation is only a sliver to indicate the other analyses that can be performed with such data. \thomas{I suggest dropping the hints on Covid altogether. It feels patched on and does not really help making our case.}




==> 06_application.tex <==
\section{Other Applications}
% \munmun{I like this section!}

The previous two sections  demonstrate that infrastructure-based coarse collocation captures some important aspects of social behaviors in students, and that these measures of behavior form a good predictor for group project success.
This presents new opportunities to harness archival network logs to scale analyses of social behaviors for larger groups, up to and including an entire campus. For instance, with an empirical understanding of how successful teams socially interact, instructors can tailor recommendations for project courses.
% Predicting the academic performance of project groups is only one of the ways campuses can support student experiences. 
This section illustrates other potential use-cases based on insights gathered from the case study.

% Unlike invasive client-based localization techniques,
% Since this method relies on logs, it can harness archival data for retrospective analyses in a way that client deployments cannot.

% \thomas{Ok, so the advantage of infrastructure-based sensing is not new and something we would need to sell here.} 

% While the method proposed in this paper does not provide the precision of fingerprinting methods it is less resource intensive because it does not require an extensive training phase \thomas{Well, we did train regression models, no?}. Traditional fingerprinting would require every building, containing multiple floors and rooms to be mapped for signal strength. Add to that the consideration of the dynamic objects that could potentially alter the signal strength  (e.g., people, new devices, solid objects). By contrast, our method provides a coarse notion of presence or proximity to an access point which is further extended to a coarse notion of co-presence. In fact, this information can reveal behaviors that indicate social interactions among individuals connected to the network. This section describes some of the applications of this that we could validate based on the ground-truth. \thomas{"could"?}



\subsection{Interaction Networks}
\label{sec:applications_interaction}
% \mehrab{general comment about this subsection. Sequencing problem for figures: figure 13 comes before firgure 12. In addition, do mention what was used to construct the network graphs. IMWUT reviewers generally ask for this kind of tool-centric details.}
% \label{sec:applications_interaction}
Social interactions are crucial to understand the physical and mental wellbeing of an individual. The lack of social interaction, or social isolation, is linked to stress, negative affect, depression and dissatisfaction~\cite{skek1991life,finch1997factor,ford1990relationship}.
% \thomas{Wow, that's quite a jump!} 
The presence of social interactions can uncover ties within a peer group, which can be helpful to understand individual perception and behavior. For instance, weak social ties are related to a lack of motivation to go to work or absenteeism~\cite{unden1996social}. Alternatively, strong social ties can also explain peer influence and its effect on alcohol, drug and tobacco use~\cite{crosnoe2004childhood}.
% also be used to infer homophily in groups which can represent congruence in perceptions and behaviors~\cite{XX}. 
% For instance, an individual can be motivated towards an activity based on their close group of associates. 
% In terms of physical wellbeing, groups with dense social interactions have increased risk of spreading contagious diseases~\cite{}. 
As a result, retrospective investigations of who a student interacts with and how these interactions evolve over a period of time can provide insights for supporting student wellbeing.

\begin{figure}[t]
    \begin{minipage}[t!]{1\columnwidth}
      \begin{subfigure}[b]{0.33\columnwidth}
        \centering
      \includegraphics[width=\columnwidth]{figures/network_jdb_2.png}
      \caption{1st week of class}
          \label{fig:net_2}
        \end{subfigure}
      \begin{subfigure}[b]{0.33\columnwidth}
        \centering
      \includegraphics[width=\columnwidth]{figures/network_jdb_8.png}
      \caption{Mid-term}
          \label{fig:net_8}
        \end{subfigure}
      \begin{subfigure}[b]{0.33\columnwidth}
        \centering
      \includegraphics[width=\columnwidth]{figures/network_jdb_12.png}
      \caption{12th week}
          \label{fig:net_12}
        \end{subfigure}
        \caption{Network graph representing time spent between individuals of 1B}
        % \thomas{Why are these results not in the results section but in this applications section?}}
        \label{fig:net_weekly}
    \end{minipage}\hfill
\end{figure}

\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{figures/network_jid_agg.png}
  \end{center}
  \caption{Network graph representing collocation time (outside class) for individuals of section 2D aggregated over the semester}
    \label{fig:net_agg}
    \vspace{-0.15in}
\end{wrapfigure}

Using the data from Section~\ref{sec:main-case-study}, we develop network graphs representing the collocation between pairs of individuals in the same section, shown in Figure~\ref{fig:net_weekly}. We compute the graphs  week-wise (excluding lecture times), with each edge depicting the duration of collocation between any pair of individuals. 
% The graphs were limited to students in the same section of a class and . 
Figure~\ref{fig:net_weekly} shows the evolution of these interaction ties between participants from Section 1B. Every node represents a participant and the color denotes project groups. Nodes that are closer illustrate individuals who spent more time collocated together.
% The distance between nodes is indirectly proportional to the duration two individuals were collocated together over that week. 
Even in the first week of class, the participants are somewhat closer to their group members than others, and this becomes more pronounced in the later weeks. However, since we consider all collocations it is evident that a participant's ties are not exclusive to their group. This makes automated methods even more valuable so as to identify these informal interactions. In some cases, members of different groups might be connected through other courses or even social circles. 


Similarly,  Figure~\ref{fig:net_agg}  represents interaction ties in section 2D aggregated over the whole study period. It reveals  the tight connection amongst some members of the red group. This particularly refers to participants 2006, 2009, and 2010. In comparison, two other group members are slightly further apart. This is explained by the disclosure during enrollment that these participants  live together. 
% Apart from them only four other participants indicated interacting with their group members outside the purposes of the academic objectives. 
This application is similar to what \citeauthor{hong2016socialprobe}, describe as relationship maps to understand intimacy between individuals~\cite{hong2016socialprobe}. By using raw association logs for an entire campus, it presents opportunities to understand where these interactions occur and semantically labels them based on the expected purpose of collocation (e.g., residential ties for roommates, academic ties for project teams, or recreational ties for parties). 


Note that our sample is limited to the 215 individuals that consented to the use of their network logs. 
% Yet, through visual analysis of the collocation based network graphs alone one can determine the tie strength between different individuals.  
More nuanced automated learning techniques can help identify social groups in a completely unsupervised way, making a compelling argument for the application to a broader cohort on campus. Accordingly, stakeholders can take actions for a cohort of individuals based on noticeable anomalies in a network, such as when someone from a cohort drops out. Another use case is when someone in a network is affected by an ailment---mental (e.g., violent incident) or physical (e.g., contagious disease)---the campus can react by securing the peers first.


% \begin{table}[t]
%     \begin{minipage}[t!]{1\columnwidth}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_before.png}
%       \caption{Before}
%           \label{fig:hmap_before}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_during.png}
%       \caption{During}
%           \label{fig:hmap_during}
%         \end{subfigure}
%       \begin{subfigure}[b]{0.33\columnwidth}
%         \centering
%       \includegraphics[width=\columnwidth]{figures/heatmap_after.png}
%       \caption{After}
%           \label{fig:hmap_after}
%         \end{subfigure}
%         \captionof{figure}{Space usage around the midterm}
%   \label{fig:hmap_space}
%     \end{minipage}\hfill
% \end{table}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/space_colloc.png}
    % \vspace{-0.1in}
  	\caption{Duration of collocations for part 1 students based on the semantic label of buildings (averaged by week).}
  	   \label{fig:space_colloc}
  	      \vspace{-0.35in}
\end{figure}

\subsection{Interaction Spaces}
% \mehrab{what does it mean to have a 0 hour after midterm in residential buildings?
% Does it indicate that there was no team deliverable after midterm and that's why students did not meet? Can we make any comments on the huge drop?
% Which category CULC or library falls under? Was there any insights for such spaces?}
% \munmun{Space utilization?}
\label{sec:applications_space}
Another approach to visually analyzing the segments identified by the pipeline is to observe where social interactions occur. 
% On simply observing the patterns of dwelling an analyst can determine where "crowding" occurs or alternatively which spaces show sparse use. 
% Figure~\ref{fig:hmap_space} shows how the dwelling changes before the midterm, during the midterm, after the midterm and in the final week. 
This can be further expanded by locating the ``collocation spaces'', which are spots on campus where individuals gather together. ~\autoref{fig:space_colloc} shows how the collocation changes before the midterm, during the midterm, after the midterm. While there is a slight increase in collocation period at academic spaces towards the end of the semester, it is most notable how the interactions in residential spaces change during the midterm. This excessive collocation could indicate groups working together to collaborate on midterm milestones or simply study for exams. Another notable aspect is the decrease of collocation duration at fraternities and sororities. This might be related to fewer parties and gatherings during midterm exams. More importantly, this data provides evidence that social interactions vary over time at different places. 

By investigating how collocation varies around specific events, say an exam, it is possible to define the purpose of spaces more dynamically. Furthermore, this can be extended to gain a better understanding of the purpose of social interactions itself. This would stem from knowledge of the space and community. Accordingly administrators could focus on facilitating better interaction in these spaces during times of collaboration. By contrast, they could also choose to carefully regulate the use of these spaces during times of social distancing~\cite{martin2020effectiveness}. 

% \thomas{So, these applications are all well and fine. However, in the absence of actual research questions (unless I am missing something, I only saw one stray hint on a "RQ2", which, however, I believe was never formally introduced) it looks all a bit unstructured. What is it that we are actually trying to research? At the moment it reads a bit like we found a cool technology (which in itself is not brandnew) and are playing around with it to see what we can find out. I know that this is not how we have been working on this project for the last n months, but that's how the paper reads like at the moment. So, my suggestion is to work on the structure of the paper and guide it through explicitly formulated (and motivated) research questions. I have also given suggestions on how to re-organize parts of the paper to make it flow better.}



\subsection{Congestion Patterns}
\label{sec:application_congestion}
% \munmun{Simply call this mobility? Maybe spatio-temporal mobility?}

% From the perspective of mental wellbeing, physical social interactions are considered constructive, however in many cases of physical wellbeing they are considered detrimental. 

Social interactions in physical spaces can lead to congestion depending on the purpose and popularity of a space. Understanding where these spaces are and when  congestion can occur can regulate gatherings for crowd-management~\cite{fan2015citymomentum,wang2016crowdwatch} and even prevent the spread of contagious diseases~\cite{martin2020effectiveness}.
% \thomas{I am confused by that last sentence, it seems contradictory in itself?} 
Therefore, campus stakeholders have an interest in identifying rooms and pathways with high pedestrian concentration. Not only could this help pre-determine bottle-necks for flock movement in cases of emergencies, it can also retroactively indicate which spaces were prone to congestion and inadvertent physical contact.  This subsection presents some observational evidence from our data showing how sections move in and out of their class room around a lecture.

\begin{table}[t!]
    \begin{minipage}[t!]{\columnwidth}
    % \begin{subfigure}[b]{\columnwidth}
    %     \centering
    %     \includegraphics[width=0.7\columnwidth]{figures/lecture_attendance.png}
    %   \end{subfigure}
    % \captionof{figure}{Attendance of 1A as detected by dwelling}
    \label{fig:lecture_attendance}
    \end{minipage}\hfill
    \begin{minipage}[t!]{\columnwidth}
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{figures/lecture_punctuality.png}
      \end{subfigure}
    \captionof{figure}{Punctuality of attending students from 1A, where the vertical red dashed lines indicate lecture times}
    \label{fig:lecture_punctuality}
    \end{minipage}\hfill
    \vspace{-0.1in}
\end{table}

As discussed in Section~\ref{sec:attendance-validation}, one of the instructors (1Q) provided us with lecture-by-lecture attendance data (46 students in Sections 1A and 1B). For Section 1A, lectures took place three times a week from 10:10-11:00, and for Section 1B, these lectures took place from 11:15-12:05. 
% In total we compute the presence of individuals for 34 lectures (this excludes the spring break period). For these lectures, over the study period we identify 83\% of students on the network to be connected to the same AP as that associated with the room and 93\% of the students to be connected to an AP in the building. Having said that, throughout the study period about 10\% of the students in the class did not connect to the network infrastructure. 
The rooms where these lectures took place were both single entry/exit. To gain a better understanding of how congested these points can get, we evaluate the arrival and exit times of the students that attend class. 
% This can be considered an under-fill/overfill error.
For entering class, we compare the earliest starting time of an individual's collocation with the designated commencement time. Similarly for exiting class, we compare the latest ending time with the lecture's expected conclusion time. The median entering time is five minutes and the median exiting time is two minutes (Figure~\ref{fig:lecture_punctuality}). These values align with the instructors' observation of typical class behavior, i.e., students are typically tardy on entry but are on time for the exit. 

Notably, our analysis considers the only students from the current class and not those who would occupy the same room for the next  or previous lecture. However, with richer data, it is possible to understand congestion points not just for class rooms but where any social interactions occur. With these findings, stakeholders could regulate the exit of students even between different rooms to avoid crowding the pathways. These can be proactive interventions to reduce the physical interactions. 
% Additionally, it can be coordinated with the lecture times of neighboring classrooms to allow smoother safer movement. This observation is only a sliver to indicate the other analyses that can be performed with such data. \thomas{I suggest dropping the hints on Covid altogether. It feels patched on and does not really help making our case.}




==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes

